Center Prediction Loss for Re-identification

The training loss function that enforces certain training sample distribution patterns plays a critical role in building a re-identification (ReID) system. Besides the basic requirement of discrimination, i.e., the features corresponding to different identities should not be mixed, additional intra-class distribution constraints, such as features from the same identities should be close to their centers, have been adopted to construct losses. Despite the advances of various new loss functions, it is still challenging to strike the balance between the need of reducing the intra-class variation and allowing certain distribution freedom. In this paper, we propose a new loss based on center predictivity, that is, a sample must be positioned in a location of the feature space such that from it we can roughly predict the location of the center of same-class samples. The prediction error is then regarded as a loss called Center Prediction Loss (CPL). We show that, without introducing additional hyper-parameters, this new loss leads to a more flexible intra-class distribution constraint while ensuring the between-class samples are well-separated. Extensive experiments on various real-world ReID datasets show that the proposed loss can achieve superior performance and can also be complementary to existing losses.

==> Center Prediction Loss for Re-identification_arxiv/Approach.tex <==
%\begin{figure}[tb]
%\begin{center}
%    \includegraphics[width=0.30\textwidth]{CPLoss.png}
%\end{center}
%\caption{The architecture of proposed CPL. The CPL is applied on the features learned from the network. The center predictor used a $2$-layer MLP to predict the anchor's center. The CPL maximizes the similarity between the predicted center and the mean of all positive (w/o anchor) features in batch. Note that the gradient only back propagation through the left branch.}
%\label{fig:CPLoss}
%\end{figure}

%\begin{figure}[tb]
%\begin{center}
%    \includegraphics[width=0.49\textwidth]{lossshape.png}
%\end{center}
%\caption{The center loss and CPL on two classes with different intra-class distribution shapes.}
%\label{fig:lossshape}
%\end{figure}


\begin{figure}[tb]
\begin{center}
    \includegraphics[width=0.45\textwidth]{architecture.pdf}
\end{center}
\caption{A default way of applying the proposed CPL. The CPL is an intra-class loss and it needs to be used with another between-class discriminative loss. In this approach, we apply a fully connection layer as an identity classifier and use the ID cross-entropy loss.}
\label{fig:cifar_architecture}
\end{figure}
 


\section{Approach}
%In this Section, we elaborate our approach. We first introduce the detail of the proposed peer prediction loss, and then use a toy example to intuitively show how it works.

In this section, we elaborate on our approach. We first introduce the detail of the proposed \textbf{C}enter \textbf{P}rediction \textbf{L}oss (CPL). Then we explain the properties of the CPL with examples. 
%Then, we provide a theoretical analysis of CPL, showing that it can be related to an upper bound of the entropy of intra-class samples. 
Finally, we provide implementation details of the CPL. 


\begin{figure}[th]
\centering 
\includegraphics[scale=0.4]{toy_loss.pdf} 
\caption{The learned $2$D embeddings ($L$-2 normalized) and their corresponding CPL (z-axis) in CIFAR-10 experiment. Different colors denote different classes. Best viewed in color. As can be seen, samples located at the class boundary tend to incur higher CPL.}
\label{fig:toy_visualization}
\end{figure}

\begin{figure*}[ht!]
\begin{center}
    \includegraphics[width=0.8\textwidth]{lossshape.pdf}
\end{center}
\caption{The center loss and the center prediction loss (CPL) on two classes with different Gaussian distributions. The class (red samples) on the left is a compact circular distribution, and the class (blue samples) on the right is an elliptic distribution with large co-variance. \textbf{Best viewed
in color}.}
\label{fig:lossshape}
\end{figure*}
\subsection{Center Prediction Loss}

%ReID is a kind of metric learning task which purpose is to make the same identity closer and different identity farther. We argue that the feature extracted from well trained network should be easy to predict its class center by a center predictor.
The proposed CPL is calculated from a set of randomly sampled same-class samples. After extracting features from a feature extractor $\phi(\cdot)$, we obtain a set of feature vectors $\{\mathbf{x}_1,\mathbf{x}_2, \cdots,\mathbf{x}_k\}$ from those intra-class samples. The CPL is defined as:
\begin{align}
\label{Fun:eq_CPL}
    \mathcal{L}_{CPL} = \min_{\theta}\mathbb{E}_{\{\mathbf{x}_1,\cdots,\mathbf{x}_k\}}\left[\sum_{i=1}^{k} \|f(\mathbf{x}_i;\theta) - \mathbf{c}_i\|_2^2\right],
\end{align} 
where $k$ is the number of intra-class samples, $f(\mathbf{x}_i;\theta)$ is the center predictor, which consists of a multi-layer perceptron (MLP) parameterized by $\theta$. $\mathbf{c}_i = \frac{1}{k-1} \sum_{j\neq i} \mathbf{x}_j$ \footnote{There might be other choices for the prediction target $\mathbf{c}_i$, e.g., the center of all same-class samples or even a randomly sampled same-class data point. We empirically find that using the center of the remaining samples leads to slightly better performance. Investigation of other target choices is provided in our ablation study.}. $\mathbb{E}$ denotes the expectation. In other words, as shown in Figure \ref{fig:cifar_architecture}, CPL is defined as the optimal predictive error from a sample to the center of the rest of same-class samples. At the first glance, CPL is very similar to the center loss, which directly requires $\mathbf{x}_i$ to be close to a learned center. However, we will show that the introduction of the center predictor (MLP) significantly changes the properties of the loss. 

\subsection{Properties of the CPL}
%\noindent\textbf{Intuitive explanation of CPL} 
The difference between CPL and traditional single-center-based intra-class loss can be well explained with the example shown in Figure \ref{fig:CPL_vs_center_loss}. As seen, for a Guassian-mixture-alike distribution shown in Figure \ref{fig:CPL_vs_center_loss}, the center loss will incur heavy penalization since the samples are not gathered around a center. In contrast, CPL will not incur a heavy loss. This is because if a sample is located at the right (or the left) side Gaussian component, it should be aware that the center of the rest same-class samples should be located in the middle. Thus, the center predictor will project a sample to the middle of the two Gaussians and lead to a small CPL. From this example, we can see that the CPL allows greater flexibility for the distribution formation. 

One potential concern of the CPL is that if it allows too much freedom for the intra-class distribution it may hurt the discrimination of between-class samples. In fact, the center prediction mechanism can automatically avoid positioning samples at the class boundary. This is because, for boundary samples,  a slight perturbation of samples will lead to a significant change of the prediction target which may jump from the center of one class sample to that of another class sample. Therefore, the center predictor will struggle to make the right prediction and in effect, it tends to incur high loss values. To validate this claim, we conduct an experiment on a subset of CIFAR-10. We set the output number of the last hidden layer to $2$ in ResNet20, which allows us to plot the features on $2$-D surface for visualization. We learn 2-dimension embeddings of samples with both an ID entropy loss and the CPL. %The model architecture is show in Figure~\ref{fig:cifar_architecture}. 
The results are shown in Figure~\ref{fig:toy_visualization} in which different colors are used to denote samples from different classes and values of CPL are shown on the $z$-axis. As can be seen, the points at the class-boundary lead to significantly higher loss values.   

We further use a simple example to illustrate how CPL works in practice. In Figure~\ref{fig:lossshape} (a), there are two Gaussian distributions with different covariance matrices, representing two classes. Then we train a center predictor for CPL, and calculate the prediction error, $e_i = \|f(\mathbf{x}_i;\theta) - \mathbf{c}_i\|_2^2$ for every data point (Note that $\mathcal{L}_{CPL} = \mathbb{E}\left[\sum e_i\right]$). Then we use the $z$-axis of each point to indicate $e_i$. To make a comparison with the center loss, we use the same visualization method but calculating $e_i = \|\mathbf{x}_i - \mathbf{c}\|_2^2$, where $\mathbf{c}$ is the respective class mean vector. The visualization results are shown in Figure~\ref{fig:lossshape} (b) and (c). From the visualization, we can see that the center loss penalizes the blue-class points much heavier than the red-class points since the former has a relatively large variance. In contrast, the CPL does not over-penalize most blue-class points. The only high loss values are incurred at the points located at the class boundary. Therefore, minimizing the CPL will not strongly force blue points to move closer to the center but push points away from the class boundary.  


%To this end, we propose the CPL, as Figure~\ref{fig:CPLoss}, it can be formulated as:
%\begin{equation}
%\resizebox{0.49\textwidth}{!}{
%\label{Fun:loss}
%$\begin{aligned}
%CPL &= \frac{1}{N}\sum_{i=1}^{N}\frac{1}{M_i}\sum_{j=1}^{M_i}Dist(MLP(feat_i_j),target_i_j)
%        &+log(\frac{1}{N}\sum_{\mu, \nu \in U}^{N}exp(-Dist(MLP(\mu),\nu))) \\
%    &\approx \frac{1}{N}\sum_{i=1}^{N}\frac{1}{M_i}\sum_{j=1}^{M_i}Dist(MLP(feat_i_j),target_i_j)
%\end{aligned}$
%}
%\end{equation}
%where $feat_i_j$ stands for the feature of $j$th image from $i$th class, $target_i_j$ is the $MLP$'s learning goal, $N$ is the class number and $M_i$ is the sample number of $i$th class. the $MLP$ is the center predictor composed of two fully connected layers. The distance metric function $Dist$ is implemented as:

%\begin{equation}
%\resizebox{0.45\textwidth}{!}{
%\label{Fun:sim}
%$Dist(center_p, target_{bn}) = 1.0 - \frac{center_p}{\parallel center_p \parallel}\cdot \frac{target_{bn}}{\parallel target_{bn} \parallel}$
%}
%\end{equation}
%where $center_p$ stands for the predicted center. The $target_{bn}$ is the mean of batch normalized positive features except anchor in the batch. In fact, if we directly use a randomly selected batch normalized positive feature as the $target_{bn}$, it still works well.

%\paragraph{Intra-class distribution shape}
%We use a simple example to illustrate how our CPL adapts to different intra-class distribution shapes. In Figure~\ref{fig:lossshape} (a), there are two gaussian distributions with different shapes, representing two classes. The class on the left is a compact circular distribution, and the class on the right is an elliptic distribution with large variance.
%We first train a center predictor for CP, and calculate the values of center loss and CPL for each sample of these two classes, and then visualize them as shown in Figure~\ref{fig:lossshape} (b) and (c). 
%We can see that center loss simply compute the loss by the distance between the sample and its class center, without considering that different class may have different distribution shapes.
%Our loss can allow different classes to have different distribution shapes on the premise of ensuring a certain degree of discrimination. Only when the position of the feature deviates from its class distribution and difficult to predict its class center, the network will be punished severely.

% \subsection{Theoretical Connection to Entropy}

% In the following, we show that the CPL can be related to an upper bound of the entropy of feature $\mathbf{x}$ which measures the uncertainty of the intra-class sample distribution.

% ~\cite{belghazi2018mutual} proved that the lower bound of KL divergence can be formulated as:


% \begin{equation}
% \label{Fun:eq_DV_1}
% D_{KL}(\mathbb{P} \parallel \mathbb{Q})  \geqslant \underset{T \in \mathcal{F} }{sup} \{\mathbb{E}_\mathbb{P} [T] - log(\mathbb{E}_\mathbb{Q}[e^T]) \}
% \end{equation}
% where $\mathbb{P}$ and $\mathbb{Q}$ are two distributions, and $\mathcal{F}$ be any class of functions $T: \Omega \rightarrow \mathbb{R}$. In particular, $T$ can be approximated by a neural network parameterized by $\theta$. From the definition of entropy and K-L divergence, we can know that $H(X) = -D_{KL}(\mathbb{P} \parallel \mathbb{U})  + const.$, where $\mathbb{P}$ is the data distribution and $\mathbb{U}$ is an uniform distribution. 

% To make the connection between the CPL and $H(X)$, we can consider a set of i.i.d sampled features $\mathcal{X} = \{X_1,X_2,\cdots,X_k\}$. The i.i.d condition states the joint probability $P(\mathcal{X}) = \prod_k P(X_k)$ and also the relationship $\frac{1}{k}H(\mathcal{X}) = H(X)$. Thus we have
% \begin{align}
%     H(X) \propto H(\mathcal{X}) = -D_{KL}(\mathbb{P}(\mathcal{X}) \parallel \mathbb{U}(\mathcal{X}))  + const.,
% \end{align}where we also extend the uniform distribution to model a set of i.i.d. sampled uniform-distributed random vectors, i.e., $U(\mathcal{X}) = \prod_k U(X_k)$, with $U(X_k)$ be an uniform distribution.
% By applying the lower bound in Eq \ref{Fun:eq_DV_1}, we have
% \begin{align}\label{eq:upper_bound}
%     \delta H(X) + \epsilon  \leq \underset{T \in \mathcal{F} }{-sup}  \left({~\mathbb{E}_{ P(\mathcal{X})} [T(\mathcal{X})]} - log({\mathbb{E}_{ U(\mathcal{X})}}[e^{T(\mathcal{X})}]) \right),
% \end{align}where both $\delta$ and $\epsilon$ are constants. If we choose a special realization of $T_{\theta}= T(\mathcal{X};\theta) = -\sum_{i=1}^{k} \|f(\mathbf{x}_i;\theta) - \mathbf{c}_i \|_2^2$ with $\mathbf{c}_i = \frac{1}{k-1} \sum_{j\neq i} \mathbf{x}_j$, %\footnote{From Eq. (7) in ~\cite{belghazi2018mutual}, we can see that when the PDF of data can be written in the Gibbs density $P(x) = \frac{1}{Z} e^{T_{\theta}}$ the bound is tight. From our discussion in Section 3.2, we can see that our $T_{\theta}$ can characterize many potential distribution patterns.}
% then the right-hand-side (RHS) of inequality \ref{eq:upper_bound} becomes 
% \begin{align}\label{eq:final_loss}
% RHS &= - \underset{T_{\theta}}{Inf}\left( -\mathbb{E}_\mathbb{P} [T] + log(\mathbb{E}_\mathbb{Q}[e^T]) \right) \nonumber \\
% &= \underset{T_{\theta}}{Inf}  \underset{\mathcal{X} \sim P(\mathcal{X})}{\mathbb{E}} [\sum_{i=1}^{k} \|f(\mathbf{x}_i;\theta) - \mathbf{c}_i \|_2^2] + \nonumber \\
% & log (\underset{\mathcal{X} \sim U(\mathcal{X})}{\mathbb{E}} [e^{-\sum_{i=1}^{k} \|f(\mathbf{x}_i;\theta) - \mathbf{c}_i \|_2^2]}). 
% \end{align} Note that the first term of Eq.\ref{eq:final_loss} is exactly the CPL. We empirically find the second term is close to a constant after the proper normalization of $\mathbf{c}_i$ and $f(\mathbf{x}_i;\theta)$ as introduced in the following section. Thus only the first term plays a major role and we can see that the proposed CPL is an approximated upper bound of $H(x)$ up to a constant scaling and shifting.

\subsection{Implementation of CPL}
To straightforwardly implement the CPL, we need first update the center predictor to find the best fit to the target and then back-propagate through the loss to the feature extractor of $\mathbf{x}_i$. However, this is computationally intractable. In practice, we \textit{jointly optimize} the parameters inside the center predictor and the other network parameters. To avoid co-adaptation of $\mathbf{x}$ and $f(\cdot)$, e.g., the network may push $\mathbf{x}$ to a very small scale for minimizing the CPL, we \textit{does not allow gradient update through $\mathbf{c}_i$.} In other words, we fix $\mathbf{c}_i$ as constant once it is calculated in the forward pass. Another important implementation detail is that we apply a batch normalization to $\mathbf{x}_i$ when calculating $\mathbf{c}_i$, namely, $\mathbf{c}_i = \frac{1}{K-1} \sum_{j\neq i} BN(\mathbf{x}_j)$. %Then we apply $l_2$ normalization to both $f(\mathbf{x}_i)$ and $\mathbf{c}_i$.
Since intra-class loss cannot be used for metric learning alone, we by default to apply it with the ID cross-entropy loss, that is, a classifier is attached to the learned embedding to categorize a sample to its given ID. Figure \ref{fig:cifar_architecture} shows the structure of the system, where we use a classifier for ID classification. 
  %$\mathbb{E}$ is the expectation. If we use $x_1 x_2 \sim P(x_1 x_2)$ as $\mathbb{P}$ and $u_1 u_2 \sim U(u_1 u_2)$ as $\mathbb{Q}$:

%\begin{equation}
%\label{Fun:eq_DV_2}
%D_{KL}(P(x_1 x_2) \parallel U(u_1 u_2))  \geqslant \underset{T \in \mathcal{F} }{sup} \mathbb{E}_P [T] - log(\mathbb{E}_U[e^T]) 
%\end{equation}
%where $U$ is a $(\beta, \beta)$ uniform sampling.
%From the relationship between entropy and KL divergence, we can know that:
%\begin{equation}
%\label{Fun:eq_DV_3}
%H(x_1 x_2) \leqslant \underset{T \in \mathcal{F} }{-sup} \underset{x_1 x_2 \sim P(x_1 x_2)} {\mathbb{E}_P [T]} + log(\underset{u_1 u_2 \sim U(u_1 u_2)}{\mathbb{E}_U}[e^T]) + \epsilon
%\end{equation}
%where $\epsilon$ is a constant.

%Then we use $-Dist(MLP(\bigcdot), \bigcdot)$ as the $T$:
%\begin{equation}
%\label{Fun:eq_DV_4}
%\begin{aligned}
%H(x_1 x_2) \leqslant &-sup \underset{x_1 x_2 \sim P(x_1 x_2)}{\mathbb{E}} [-Dist(MLP(x_1),x_2)] \\
 %                    &+ log(\underset{u_1 u_2 \sim U(u_1 u_2)}{\mathbb{E}}[  e^{-Dist(MLP(u_1),u_2)}]) + \epsilon \\
 %                    &\approx Inf \underset{x_1 x_2 \sim P(x_1 x_2)}{\mathbb{E}} [Dist(MLP(x_1),x_2)] + \omega 
%\end{aligned}
%\end{equation}
%where $\omega$ is a constant.

%Now, It is Eq~\ref{Fun:loss}. And we can found that minimizing the formula~\ref{Fun:eq_DV_4} on the right is actually minimizing the upper bound of $x$'s entropy.


%\subsection{Cifar-10 Toy Experiment}
%In this section, a toy example on a subset of cifar-10~\cite{krizhevsky2009learning} dataset is presented. Similar to the toy example in ~\cite{wen2016discriminative}, we reduce the output number of the last hidden layer to $2$ in ResNet20, which can directly plot the features on $2$-D surface for visualization. The model architecture. And for better visualization, we randomly selected three classes as the subset of cifar-10.

%We trained the model with the combination of softmax loss and CPL for $100$ epochs and then visualized the features. As Figure~\ref{fig:toy_visualization} (a) shows, the predictor can easily predict the center area if the feature within the scope of the class.
%On the contrary, if the feature located outside of its class scope, it will be difficult to predict its center. As Figure~\ref{fig:toy_visualization} (b) shows, it will get a huge punish from the CPL, forcing the network to locate the feature to be in the position where is easy to predict its class center.
%As a result, each class will optimize its own scope according to the feature distribution adaptively.

%Note that, the scope of the green class is more than twice that of the blue class, it shows that different classes have different degrees of intra-class distribution, and fixed intra-class margin~\cite{wang2019ranked} may not be suitable for all classes.

Note that the proposed CPL can be simply plugged into any deep metric learning system as an additional loss function. We present the pseudo-code of the CPL in Algorithm \ref{alg}. 
\begin{center}
    \vskip -0.1in
        \begin{algorithm}[H]
            \caption{Applying Center Prediction Loss for ReID systems}
            \label{alg}
        \begin{algorithmic}[1]
            \STATE {\bfseries Input:} $\mathcal{D}$
            \STATE Randomly initialize feature extractor $\phi(\cdot;\lambda)$ and center predictor (MLP) $f(\cdot;\theta)$
            
            \FOR{$t=0$ {\bfseries to} $T$}
            \STATE Sample $P$ IDs with $K$ images per ID from $\mathcal{D}$. Extracting their features as $\{\{ \mathbf{x}_i^c \}_{i=1}^K\}\}_{c=1}^P$  
            \STATE Compute $\mathbf{c}_i^c = \frac{1}{K-1} \sum_{j=1, j\neq i}^{K}  BN(\mathbf{x}_j^c)$
            \STATE Compute loss $\mathcal{L}_{CPL} = \sum_c \frac{1}{K} \sum_i \|f(\mathbf{x}_i^c;\theta) - \mathbf{c}_i\|_2^2$ 
            \STATE Calculate ID cross-entropy loss $\mathcal{L}_{ce}$ for samples
            \STATE Update both $\theta$ and $\lambda$ with by back-propagate $\mathcal{L}_{CPL} + \lambda \mathcal{L}_{ce}$ via SGD.
            \ENDFOR
 
        \end{algorithmic}
        \end{algorithm}
\end{center}


==> Center Prediction Loss for Re-identification_arxiv/Conclusion.tex <==
\section{Conclusion}
In this work, we propose a new loss called the center prediction loss to strike the balance between intra-class variation reduction and flexible intra-class distribution modeling. The loss encourages a sample to be positioned in a location such that from it we can roughly predict the center of the same-class samples. 
We show that the proposed CPL allows greater freedom in data distribution families and it can also preserve the discrimination of learned embedding by avoiding positioning samples around the class boundaries. 
%To this end, we propose a learnable Center Prediction Loss in ReID task, it can adaptively optimize the scope of each class in the embedding space with-out using margin. It can preserve different intra-class distributions with different shapes.
%Moreover, we show that CPL has a theoretical connection with the entropy of intra-class features. Through our derivation, we show that the CPL can be roughly seen as an upper-bound of entropy. 
%show that the proposed loss can be viewed as an approximated upper bound of the entropy of intra-class samples.
We carried out extensive experiments on various real-world ReID datasets to demonstrate that the proposed loss is a powerful alternative to many existing metric learning losses. Also, it can be complementary to these losses and achieve higher performance.


%can replace the traditional metric learning loss in ReID task to improve the performance, and it can achieve higher performance when working together with them.


==> Center Prediction Loss for Re-identification_arxiv/Experiment.tex <==
\begin{table*}[tb]
		\centering
		\footnotesize
	\scalebox{0.98}{
    \begin{tabular}{crrrrrrrrrrr}
    	\hline
    	\multicolumn{1}{c}{\multirow{3}[4]{*}{Method}} & \multicolumn{4}{c}{CUHK03} & \multicolumn{2}{c}{\multirow{2}[2]{*}{Market1501}} & \multicolumn{2}{c}{\multirow{2}[2]{*}{Duke}} & \multicolumn{2}{c}{\multirow{2}[2]{*}{MSMT17}} \bigstrut[t]\\
    	\multicolumn{1}{c}{} & \multicolumn{2}{c}{Labeled} & \multicolumn{2}{c}{Detected} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} \bigstrut[b]\\
    	\cline{2-11} \multicolumn{1}{c}{} & \multicolumn{1}{c}{Rank-1} & \multicolumn{1}{c}{mAP} & \multicolumn{1}{c}{Rank-1} & \multicolumn{1}{c}{mAP} & \multicolumn{1}{c}{Rank-1} & \multicolumn{1}{c}{mAP} & \multicolumn{1}{c}{Rank-1} & \multicolumn{1}{c}{mAP} & \multicolumn{1}{c}{Rank-1} & \multicolumn{1}{c}{mAP} \bigstrut\\
    	\hline
    	 
    	\multicolumn{1}{l}{IDE~\cite{sun2017beyond}} & \multicolumn{1}{c}{43.8 } & \multicolumn{1}{c}{38.9 } & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{85.3 } & \multicolumn{1}{c}{68.5 } & \multicolumn{1}{c}{73.2 } & \multicolumn{1}{c}{52.8 } & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{- } \bigstrut[t]\\ 
    	%\multicolumn{1}{l}{Gp-reid~\cite{almazan2018re}} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{92.2 } & \multicolumn{1}{c}{81.2 } & \multicolumn{1}{c}{85.2 } & \multicolumn{1}{c}{72.8 } & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{- }\bigstrut[t]\\
    	%\hline
    	 
    	\multicolumn{1}{l}{MGCAM~\cite{song2018mask}} & \multicolumn{1}{c}{50.1 } & \multicolumn{1}{c}{50.2 } & \multicolumn{1}{c}{46.7 } & \multicolumn{1}{c}{46.9 } & \multicolumn{1}{c}{83.8 } & \multicolumn{1}{c}{74.3 } & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-}& \multicolumn{1}{c}{-} & \multicolumn{1}{c}{- } \bigstrut[t]\\
    	%\multicolumn{1}{l}{MaskReID~\cite{qi2018maskreid}} &  \multicolumn{1}{c}{-}  &  \multicolumn{1}{c}{-}  &  \multicolumn{1}{c}{-}  &  \multicolumn{1}{c}{-}  & \multicolumn{1}{c}{90.0 } & \multicolumn{1}{c}{70.3 } & \multicolumn{1}{c}{78.9 } & \multicolumn{1}{c}{61.9 }& \multicolumn{1}{c}{-} & \multicolumn{1}{c}{- } \bigstrut[t]\\
    	\multicolumn{1}{l}{AACN~\cite{xu2018attention}} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{85.9 } & \multicolumn{1}{c}{66.9 } & \multicolumn{1}{c}{76.8 } & \multicolumn{1}{c}{59.3 } & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{- }\bigstrut[t]\\
    	\multicolumn{1}{l}{SPReID~\cite{kalayeh2018human}} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{92.5 } & \multicolumn{1}{c}{81.3 } & \multicolumn{1}{c}{84.4 } & \multicolumn{1}{c}{71.0 }  & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{- }\bigstrut[t]\\
    	%\cline{2-10}       
    	\multicolumn{1}{l}{HA-CNN~\cite{li2018harmonious}} & \multicolumn{1}{c}{44.4 } & \multicolumn{1}{c}{41.0 } & \multicolumn{1}{c}{41.7 } & \multicolumn{1}{c}{38.6 } & \multicolumn{1}{c}{91.2 } & \multicolumn{1}{c}{75.7 } & \multicolumn{1}{c}{80.5 } & \multicolumn{1}{c}{63.8 } & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{- }\bigstrut[t]\\
    	\multicolumn{1}{l}{DuATM~\cite{si2018dual}} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{91.4 } & \multicolumn{1}{c}{76.6 } & \multicolumn{1}{c}{81.8 } & \multicolumn{1}{c}{64.6 }  & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{- }\bigstrut[t]\\
    	\multicolumn{1}{l}{Mancs~\cite{wang2018mancs}} & \multicolumn{1}{c}{69.0 } & \multicolumn{1}{c}{63.9 } & \multicolumn{1}{c}{65.5 } & \multicolumn{1}{c}{60.5 } & \multicolumn{1}{c}{93.1 } & \multicolumn{1}{c}{82.3 } & \multicolumn{1}{c}{84.9 } & \multicolumn{1}{c}{71.8 } & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{- }\bigstrut[t]\\
    	%\hline
    	\multicolumn{1}{l}{HPM~\cite{fu2019horizontal}} & \multicolumn{1}{c}{63.9 } & \multicolumn{1}{c}{57.5 } & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{94.2 } & \multicolumn{1}{c}{82.7 } & \multicolumn{1}{c}{86.6 } & \multicolumn{1}{c}{74.3 }& \multicolumn{1}{c}{-} & \multicolumn{1}{c}{- } \bigstrut[t]\\
    	\multicolumn{1}{l}{DSA-reID~\cite{zhang2019densely}} & \multicolumn{1}{c}{78.9 } & \multicolumn{1}{c}{75.2 } & \multicolumn{1}{c}{78.2} & \multicolumn{1}{c}{73.1 } & \multicolumn{1}{c}{\textbf{95.7 }} & \multicolumn{1}{c}{87.6 } & \multicolumn{1}{c}{86.2 } & \multicolumn{1}{c}{74.3 }& \multicolumn{1}{c}{-} & \multicolumn{1}{c}{- } \bigstrut[t]\\
    	\multicolumn{1}{l}{IANet~\cite{zhang2019densely}} & \multicolumn{1}{c}{- } & \multicolumn{1}{c}{- } & \multicolumn{1}{c}{- } & \multicolumn{1}{c}{- } & \multicolumn{1}{c}{94.4 } & \multicolumn{1}{c}{83.1 } &
    	\multicolumn{1}{c}{- } & \multicolumn{1}{c}{- } &
    	\multicolumn{1}{c}{75.5 } & \multicolumn{1}{c}{46.8} \bigstrut[t]\\
    	\multicolumn{1}{l}{JDGL~\cite{fu2019horizontal}} & \multicolumn{1}{c}{- } & \multicolumn{1}{c}{- } & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{94.8 } & \multicolumn{1}{c}{86.0 } &
    	\multicolumn{1}{c}{-} & \multicolumn{1}{c}{- } &
    	\multicolumn{1}{c}{77.2 } & \multicolumn{1}{c}{52.3 } \bigstrut[t]\\
    	\multicolumn{1}{l}{OSNet~\cite{fu2019horizontal}} & \multicolumn{1}{c}{- } & \multicolumn{1}{c}{- } & \multicolumn{1}{c}{72.3} & \multicolumn{1}{c}{67.8} & \multicolumn{1}{c}{94.8 } & \multicolumn{1}{c}{84.9 } & \multicolumn{1}{c}{- } & \multicolumn{1}{c}{- } & \multicolumn{1}{c}{78.7 } & \multicolumn{1}{c}{52.9 } \bigstrut[t]\\
        %\multicolumn{1}{l}{SCSN CVPR20 4 stage)~\cite{chen2020salience}} & \multicolumn{1}{c}{86.80 } & \multicolumn{1}{c}{84.00} & \multicolumn{1}{c}{84.70} & \multicolumn{1}{c}{81.00} & \multicolumn{1}{c}{92.40 } & \multicolumn{1}{c}{88.30} & \multicolumn{1}{c}{91.00} & \multicolumn{1}{c}{79.00} & \multicolumn{1}{c}{83.80 } & \multicolumn{1}{c}{58.50 } \bigstrut[t]\\
        %\multicolumn{1}{l}{(Baseline-SNR CVPR20 )~\cite{jin2020style}} & \multicolumn{1}{c}{- } & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{93.40 } & \multicolumn{1}{c}{82.3} & \multicolumn{1}{c}{85.50} & \multicolumn{1}{c}{73.20} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{- } \bigstrut[t]\\
        \multicolumn{1}{l}{HOReid~\cite{wang2020high}} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{94.2 } & \multicolumn{1}{c}{84.9} & \multicolumn{1}{c}{86.9} & \multicolumn{1}{c}{75.6} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{- } \bigstrut[t]\\
        
        \multicolumn{1}{l}{ISP~\cite{zhu2020identity}} & \multicolumn{1}{c}{76.5} & \multicolumn{1}{c}{74.1} & \multicolumn{1}{c}{75.2} & \multicolumn{1}{c}{71.4} & \multicolumn{1}{c}{95.3 } & \multicolumn{1}{c}{\emph{88.6}} & \multicolumn{1}{c}{\textbf{89.6}} & \multicolumn{1}{c}{\textbf{80.0}} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{- } \bigstrut[t]\\
    	\hline
    	\multicolumn{1}{l}{AlignedReID$^{\dag}$~\cite{luo2019alignedreid}} & \multicolumn{1}{c}{53.8} & \multicolumn{1}{c}{49.0} & \multicolumn{1}{c}{50.5} & \multicolumn{1}{c}{45.6} & \multicolumn{1}{c}{84.9} & \multicolumn{1}{c}{68.0} & \multicolumn{1}{c}{76.5} & \multicolumn{1}{c}{59.6}& \multicolumn{1}{c}{58.8} & \multicolumn{1}{c}{33.7}  \bigstrut[t]\\
    	\multicolumn{1}{l}{AlignedReID + CPL} & \multicolumn{1}{c}{55.6} & \multicolumn{1}{c}{50.1} & \multicolumn{1}{c}{52.4} & \multicolumn{1}{c}{47.0} & \multicolumn{1}{c}{85.2} & \multicolumn{1}{c}{69.5} & \multicolumn{1}{c}{79.0} & \multicolumn{1}{c}{61.3}& \multicolumn{1}{c}{62.7} & \multicolumn{1}{c}{36.5}  \bigstrut[b]\\
    	\hline
    	%\multicolumn{1}{l}{MGN$^{\dag}$~\cite{wang2018learning}} & \multicolumn{1}{c}{x } & \multicolumn{1}{c}{x } & \multicolumn{1}{c}{x } & \multicolumn{1}{c}{x } & \multicolumn{1}{c}{x } & \multicolumn{1}{c}{x } & \multicolumn{1}{c}{x } & \multicolumn{1}{c}{x } \bigstrut[t]\\
    	%\multicolumn{1}{l}{MGN + CPL} & \multicolumn{1}{c}{xx } & \multicolumn{1}{c}{xx } & \multicolumn{1}{c}{xx } & \multicolumn{1}{c}{xx } & \multicolumn{1}{c}{xx } & \multicolumn{1}{c}{xx } & \multicolumn{1}{c}{xx } & \multicolumn{1}{c}{xx } \bigstrut[b]\\
    	\multicolumn{1}{l}{BoT$^{\dag}$~\cite{luo2019bag}} & \multicolumn{1}{c}{68.9} & \multicolumn{1}{c}{66.8} & \multicolumn{1}{c}{65.2} & \multicolumn{1}{c}{62.9} & \multicolumn{1}{c}{93.7} & \multicolumn{1}{c}{84.9} & \multicolumn{1}{c}{85.2} & \multicolumn{1}{c}{75.1} & \multicolumn{1}{c}{73.8} & \multicolumn{1}{c}{50.1}  \bigstrut[t]\\
    	\multicolumn{1}{l}{BoT + CPL} &  \multicolumn{1}{c}{71.9} & \multicolumn{1}{c}{69.6} & \multicolumn{1}{c}{68.3} & \multicolumn{1}{c}{65.9} & \multicolumn{1}{c}{94.7} & \multicolumn{1}{c}{87.0} & \multicolumn{1}{c}{87.3} & \multicolumn{1}{c}{76.4} & \multicolumn{1}{c}{75.0} & \multicolumn{1}{c}{51.8} \bigstrut[b]\\
    	\hline
    	\multicolumn{1}{l}{RGA$^{\dag}$~\cite{zhang2020relation}} & \multicolumn{1}{c}{\emph{81.1}} & \multicolumn{1}{c}{\emph{77.2}} & \multicolumn{1}{c}{\emph{78.9}} & \multicolumn{1}{c}{\emph{75.0}} & \multicolumn{1}{c}{95.2} & \multicolumn{1}{c}{88.4} & \multicolumn{1}{c}{88.7} & \multicolumn{1}{c}{78.4} & \multicolumn{1}{c}{\emph{79.9}} & \multicolumn{1}{c}{\emph{56.7}} \bigstrut[t]\\
    	\multicolumn{1}{l}{RGA + CPL} & \multicolumn{1}{c}{\textbf{82.5}} & \multicolumn{1}{c}{\textbf{78.3}} & \multicolumn{1}{c}{\textbf{80.9}} & \multicolumn{1}{c}{\textbf{76.8}} & \multicolumn{1}{c}{\emph{95.5}} & \multicolumn{1}{c}{\textbf{88.8}} & \multicolumn{1}{c}{\emph{89.0}} & \multicolumn{1}{c}{\emph{78.8}} & \multicolumn{1}{c}{\textbf{81.4}} & \multicolumn{1}{c}{\textbf{57.8}} \bigstrut[b]\\

    	\hline
    \end{tabular}
    }

	\caption{Performance (\%) comparisons with the state-of-the-arts on CUHK03, Market1501, Duke and MSMT17. ``\dag'' means by our implementation. \textbf{Bold} and \emph{Italic} fonts represent the best and second best performance respectively.}
	\label{tab:SOTA_person}
\end{table*}


\begin{table}[tb]
	\begin{center}
		\scalebox{0.73}{
			\begin{tabular}{c|cc|cc}
				\hline
				\multicolumn{1}{c|}{\multirow{2}{*}{Method}} & \multicolumn{2}{c|}{VeRi-776} &  \multicolumn{2}{c}{VehicleID (Large)} \\ \cline{2-5} 
				\multicolumn{1}{c|}{} & \multicolumn{1}{c}{Rank-1} & \multicolumn{1}{c}{mAP}  & \multicolumn{1}{|c}{Rank-1} & \multicolumn{1}{c}{mAP}  \\
				\hline \hline
				% ~\cite{khorramshahi2019dual}
				AAVER$^*$ [Khorramshahi et al., 2019] & $89.0$  &  $61.2$ &$63.5$ & $-$\\
				%VANet~\cite{Chu_2019_ICCV}$^*$ & $66.3$ & $89.8$ & $-$ & $\mathbf{80.4}$\\
				% ~\cite{he2019part}
				PRND$^{*\ddag}$ [He et al., 2019] & $94.3$ & $74.3$ & $74.2$ & $-$\\
				\hline
				% ~\cite{bai2018group}
				GS-TRE(ResNet50) [Bai et al., 2018] & $-$ & $-$ & $-$ & $78.8$\\
				% ~\cite{lou2019veri}
				FDA-Net [Lou et al., 2019b] & $84.3$ & $55.5$ & $55.5$ & $61.8$\\
				% ~\cite{lou2019embedding}
				EALN [Lou et al., 2019a] & $84.4$ & $57.4$ & $69.3$ & $71.0$\\
				% ~\cite{alfasly2019variational}
				Mob.VFL [Alfasly et al., 2019] & $87.2$ & $58.1$ & $67.4$ & $-$\\
				% ~\cite{zhu2019vehicle}
				QD-DLP [Zhu et al., 2019] & $88.5$ & $61.8$ & $64.1$ & $68.4$\\
				% ~\cite{Chen_2019_ICCV}
				DMML [Chen et al., 2019] & $91.2$ & $70.1$ & $67.7^{\dag}$ & $72.4^{\dag}$\\
				% ~\cite{lin2019multi}   [Lin et al., 2019]
				MRL~\cite{lin2019multi}$^{\ddag}$& $94.3$ & $78.5$ & $\mathbf{78.4}$ & $\emph{81.2}$\\
				% 
				SAVER$^{\ddag}$~\cite{ECCV2020Devil}& $\mathbf{96.4}$ & $\emph{79.6}$ & $75.3$ & $-$\\
				\hline
				BoT$^{\dag}$~\cite{luo2019bag} & $94.7$ & $79.3$ & $75.5$ & $81.0$\\
				BoT + CPL & $\emph{96.0}$ & $\mathbf{80.6}$ & $\emph{76.7}$ & $\mathbf{82.3}$\\
				\hline
			\end{tabular}
	  	}
	\end{center}
	\caption{Comparison with state of the art methods on VeRi-776 and VehicleID (in \%). ``*'' indicates models trained with extra annotations such as keypoints or viewpoints. ``\dag'' means by our implementation. The input image size is $224\times 224$ by default except the methods with ``\ddag''. \textbf{Bold} and \emph{Italic} fonts represent the best and second best performance respectively. }
	\label{tab:SOTA_vehicle}
\vspace{-1em}
\end{table}


\begin{table}[tb]
\begin{center}
\scalebox{0.85}{
\begin{tabular}{c|cc}
\hline
\multicolumn{1}{c|}{Method} & Rank-1 & Rank-5 \\ \hline \hline
OIFE(Single Branch)* & $24.6$ & $51.0$ \\
Siamese-Visual* & $30.5$ & $57.3$ \\
MSVF~\cite{kanaci2018vric}& $46.6$ & $65.6$ \\
%MSVF [Kanacı et al., 2018] & $46.6$ & $65.6$ \\
CRAD~\cite{li2020cross}& $50.1$ & $68.2$ \\
%CRAD [Li et al., 2020]& $50.1$ & $68.2$ \\
BW~\cite{kumar2020strong}& $69.1$ & $90.5$ \\
%BW [Kumar et al., 2020]& $69.1$ & $90.5$ \\
\hline
BoT$^{\dag}$~\cite{luo2019bag} & $74.3$ & $90.3$ \\ 
BoT + CPL    & $\mathbf{76.6}$ & $\mathbf{91.8}$ \\
\hline
\end{tabular}
}
 \caption{Comparison with state-of-the-art methods on VRIC (in \%). \textbf{Bold} fonts represent the best performance. ``\dag'' means by our implementation. ``*'' refers to results represented in MSVF.}
 \label{tab:SOTA_VRIC}
\end{center}
\vspace{-1mm}
\end{table}


\section{Experiments}

\subsection{Datasets}
We conduct extensive experiments on four public person ReID datasets, $i.e.$, Market1501~\cite{iccv15zheng}, Duke~\cite{iccv17duke}, CUHK03~\cite{cvpr14cuhk} and MSMT17~\cite{cvpr18msmt}. We also verify the effectiveness of our loss on three largescale vehicle ReID datasets, $i.e.$, VeRi-776~\cite{liu2016veri776}, VehicleID~\cite{liu2016vehicleid} and VRIC~\cite{kanaci2018vric}. The Cumulative Match Curve (CMC) at Rank-1 and the mean Average Precision (mAP) are used as the evaluation criteria.

\subsection{Implementation Details}
Unless specified otherwise, we use BOT~\cite{luo2019bag} as the baseline by default. We didn't utilize label smooth, test with flip and re-ranking. All the experiments use ResNet50 as the backbone. The center predictor is a two-layer MLP, whose hidden layer is $512$-dimension. The person images were resized to $256 \times 128$ and vehicle images were resized to $224 \times 224$. The batch size is $64$ ($4$ images/ID and $16$ IDs). The model is trained $120$ epochs and the learning rate is initialized to $3.5\times 10^{-4}$ and divided by $10$ at the $40$th epoch and $70$th epoch.
The detailed implementation of other methods follows the settings in their respective papers.



\subsection{CPL with SOTA Methods}
In this section we evaluate the performance of our proposed loss by incorporating it into several state-of-the-art approaches.
For person ReID benchmarks, we apply CPL on \cite{luo2019alignedreid,luo2019bag,zhang2020relation} that already use ID cross-entropy loss and hard triplet loss. The results are shown in Table~\ref{tab:SOTA_person}. It is clear that our CPL can further improve the performance of several SOTA methods on four public person ReID datasets.

To further validate the effectiveness of our loss, we also conduct experiments on three vehicle datasets.
Although BoT~\cite{luo2019bag} is originally designed for person ReID, applying it to vehicle ReID is straightforward given their similar pipelines. We resize the image size from $256 \times 128$ to $224 \times 224$ in vehicle ReID. As shown in Table~\ref{tab:SOTA_vehicle} and Table~\ref{tab:SOTA_VRIC}, our method yields a consistent performance gain over these vehicle datasets in different degrees, ranging from $1.2\%$ to $2.3\%$ on Rank-1.


\begin{table*}[tb]
\begin{center}
    \begin{tabular}{crrrrrrrrrrr}
    	\hline
    	\multicolumn{1}{c}{\multirow{3}[4]{*}{Method}} & \multicolumn{4}{c}{CUHK03} & \multicolumn{2}{c}{\multirow{2}[2]{*}{Market1501}} & \multicolumn{2}{c}{\multirow{2}[2]{*}{Duke}} & \multicolumn{2}{c}{\multirow{2}[2]{*}{MSMT17}} \bigstrut[t] \\
    	\multicolumn{1}{c}{} & \multicolumn{2}{c}{Labeled} & \multicolumn{2}{c}{Detected} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} \bigstrut[b] \\
    	\cline{2-11} \multicolumn{1}{c}{} & \multicolumn{1}{c}{Rank-1} & \multicolumn{1}{c}{mAP} & \multicolumn{1}{c}{Rank-1} & \multicolumn{1}{c}{mAP} & \multicolumn{1}{c}{Rank-1} & \multicolumn{1}{c}{mAP} & \multicolumn{1}{c}{Rank-1} & \multicolumn{1}{c}{mAP} & \multicolumn{1}{c}{Rank-1} & \multicolumn{1}{c}{mAP} \bigstrut \\
    	\hline
    	\multicolumn{1}{l}{Baseline (ID cross-entropy only)} & \multicolumn{1}{c}{65.71} & \multicolumn{1}{c}{63.36} & \multicolumn{1}{c}{63.93} & \multicolumn{1}{c}{60.11} & \multicolumn{1}{c}{93.29 } & \multicolumn{1}{c}{83.06 } & \multicolumn{1}{c}{84.34} & \multicolumn{1}{c}{72.87} & \multicolumn{1}{c}{71.38 } & \multicolumn{1}{c}{47.08 } \bigstrut[t] \\
    	\multicolumn{1}{l}{Baseline + CPL} & \multicolumn{1}{c}{69.57} & \multicolumn{1}{c}{68.17} & \multicolumn{1}{c}{67.29} & \multicolumn{1}{c}{65.36} & \multicolumn{1}{c}{94.06} & \multicolumn{1}{c}{86.09} & \multicolumn{1}{c}{86.27} & \multicolumn{1}{c}{75.34}& \multicolumn{1}{c}{74.51} & \multicolumn{1}{c}{50.68} \bigstrut[b] \\
    	\hline

    	\multicolumn{1}{l}{Baseline + Center~\cite{wen2016discriminative}} & \multicolumn{1}{c}{64.57} & \multicolumn{1}{c}{63.03} &  \multicolumn{1}{c}{62.57} & \multicolumn{1}{c}{59.65} & \multicolumn{1}{c}{92.87} & \multicolumn{1}{c}{82.78} & \multicolumn{1}{c}{83.48} & \multicolumn{1}{c}{72.52}& \multicolumn{1}{c}{70.92} & \multicolumn{1}{c}{46.37} \bigstrut[t] \\
    	\multicolumn{1}{l}{Baseline + Center + CPL} & \multicolumn{1}{c}{67.36} & \multicolumn{1}{c}{66.28} & \multicolumn{1}{c}{66.43} & \multicolumn{1}{c}{63.96} & \multicolumn{1}{c}{93.41} & \multicolumn{1}{c}{84.70} & \multicolumn{1}{c}{85.14} & \multicolumn{1}{c}{74.89} & \multicolumn{1}{c}{72.51} & \multicolumn{1}{c}{49.27}\bigstrut[t] \\
    	\hline
    	
    	\multicolumn{1}{l}{Baseline + RLL~\cite{wang2019ranked}} & \multicolumn{1}{c}{67.86} & \multicolumn{1}{c}{66.71} & \multicolumn{1}{c}{63.79} & \multicolumn{1}{c}{62.84} & \multicolumn{1}{c}{93.79} & \multicolumn{1}{c}{84.65} & \multicolumn{1}{c}{86.18} & \multicolumn{1}{c}{75.25} & \multicolumn{1}{c}{72.45} & \multicolumn{1}{c}{48.80} \bigstrut[t] \\
    	\multicolumn{1}{l}{Baseline + RLL + CPL} & \multicolumn{1}{c}{71.29} & \multicolumn{1}{c}{\textbf{69.83}} & \multicolumn{1}{c}{\textbf{68.71}} & \multicolumn{1}{c}{\textbf{66.98}} & \multicolumn{1}{c}{94.09} & \multicolumn{1}{c}{86.21} & \multicolumn{1}{c}{86.58} & \multicolumn{1}{c}{76.05} & \multicolumn{1}{c}{73.23} & \multicolumn{1}{c}{50.25}\bigstrut[t] \\
    	\hline
    	
    	\multicolumn{1}{l}{Baseline + Triplet~\cite{schroff2015facenet}} & \multicolumn{1}{c}{68.93} & \multicolumn{1}{c}{66.82} & \multicolumn{1}{c}{65.21} & \multicolumn{1}{c}{62.90} & \multicolumn{1}{c}{93.68} & \multicolumn{1}{c}{84.90} & \multicolumn{1}{c}{85.19} & \multicolumn{1}{c}{75.07}& \multicolumn{1}{c}{73.80} & \multicolumn{1}{c}{50.07} \bigstrut[t] \\
    	\multicolumn{1}{l}{Baseline + Triplet + CPL} & \multicolumn{1}{c}{\textbf{71.86}} & \multicolumn{1}{c}{69.58} & \multicolumn{1}{c}{68.29} & \multicolumn{1}{c}{65.91} & \multicolumn{1}{c}{\textbf{94.66}} & \multicolumn{1}{c}{\textbf{86.96}} & \multicolumn{1}{c}{\textbf{87.34}} & \multicolumn{1}{c}{\textbf{76.41}}& \multicolumn{1}{c}{\textbf{75.00}} & \multicolumn{1}{c}{\textbf{51.84}} \bigstrut[t] \\
    	\hline
    	
    \end{tabular}
    \caption{The CPL is complementary to other loss functions. The baseline is BoT with ID cross-entropy loss only. \textbf{Bold} fonts represent the best performance (in \%).}
	\label{tab:losses}
\end{center}
\end{table*}



\begin{table}[tb]
    \begin{center}
     \scalebox{0.78}{
    \begin{tabular}{c|cccc}
    \hline
    \cline{2-5}
    & Market1501 & Duke & CUHK03(L) & MSMT17 \\
    \hline\hline
    Random point. & $86.30$ & $76.39$ & $\textbf{69.71}$ & $51.15$ \\
    Farthest point    & $86.76$ & $76.18$ & $69.56$ & $51.57$ \\
    Sample mean & $86.59$ & $76.18$ & $69.33$ & $51.46$ \\
    Leave-one-out mean & $\textbf{86.96}$ & $\textbf{76.41}$ &$69.58$  & $\textbf{51.84}$ \\
    \hline
    \end{tabular}
    }
    \caption{The mAP (\%) comparison with different predictor target. \textbf{Bold} fonts represent the best performance.}
     \label{tab:target}
    \end{center}
\end{table}


\subsection{Ablation Study}
In this section, we perform an ablation study on several key factors.
Unless specified otherwise, the default setting in the experiment is BoT~\cite{luo2019bag} trained with ID cross-entropy loss, triplet loss, and our proposed CPL. %BoT investigates a large number of useful tricks, such as hard mining, warmup, random erasing, et al. 

\paragraph{Target of predictor}
In the CPL, the MLP predicts the center of the remaining same-class samples. However, theoretically, it is possible to use other prediction targets. In this ablation study, we conduct experiments to evaluate several alternatives. They are: (1) a randomly chosen same-class point (Random point), (2) a sample which is farthest to the current point (Farthest point), and (3) average of all the same-class samples (Sample mean). We compare them with the target used in the CPL, i.e., an average of remaining same-class samples (Leave-one-out mean). 

%If random positive or hard positive used as the $target$, the predictor's learning goal can be viewed as the average representation over the distribution of intra-class~\cite{chen2020exploring}. Because only in this way can the loss expectation be minimized.
The results are shown in Table~\ref{tab:target}. We can see that the performance of these four different ways is comparable, and using the mean of remaining same-class samples is slightly better than others, so we use it as the target in CPL by default.


%\paragraph{Impact of loss weight}
%The loss weight is usually important when there are multiple loss functions work together.
%We conduct experiments on person ReID task to evaluate the influence of loss weight of CPL when working with the baseline. The baseline is BoT~\cite{luo2019bag} with softmax and triplet loss. We vary the loss weight $\beta$ of CPL from $0.05$ to $5.0$ in Eq. (\ref{eq:weight}) and the results are shown at Table~\ref{tab:lossweight}.
%\begin{equation}
%\label{eq:weight}
%L_{total} = L_{softmax} + L_{triplet} + \beta * L_{total} 
%\end{equation}

% \begin{table}[tb]
%     \begin{center}
%     \scalebox{0.9}{
%     \begin{tabular}{c|cccc}
%     \hline
%     \cline{2-5}
%     loss weight & CUHK03(L) &Market1501 & Duke &  MSMT17 \\
%     \hline\hline
%     $\beta=0.05$ & $66.1$ & $85.3$ & $75.1$ & $50.8$ \\
%     $\beta=0.1$  & $67.6$ & $85.2$ & $75.4$ & $51.0$ \\
%     $\beta=0.5$  & $68.9$ & $86.2$ & $76.0$ & $51.5$ \\
%     $\beta=1.0$  & $\textbf{69.6}$ & $\textbf{87.0}$ & $\textbf{76.4}$ & $\textbf{51.8}$ \\
%     $\beta=2.0$  & $69.2$ & $\textbf{87.0}$ & $76.3$ & $51.6$ \\
%     $\beta=5.0$  & $67.0$ & $85.5$ & $72.6$ & $49.0$ \\
%     \hline
%     \end{tabular}
%     }
%     \caption{Effect of weighting factor $\beta$ of CPL when working together with softmax loss and triplet loss (in \%). \textbf{Bold} fonts represent the best performance.}
%     \label{tab:lossweight}
%     \end{center}
% \end{table}

%\subsection{center as query}

 
\paragraph{Complementarity of the CPL and other losses}
As mentioned in the introduction, the CPL is an intra-class loss that encourages certain distribution patterns of the same-class samples. It usually works with other loss functions. In this section, we conduct experiments to combine the CPL with other loss functions. The purpose of this experiment to check if the CPL can be beneficial in addition to the existing loss functions. 

%Traditional metric learning losses generally learns discriminative features by constraining the distance between samples or between samples and class centers.
%Our CPL use the property of center predictivity to force the network to learn the discriminative feature.
%Different consideration lead to the possible complementarity between our loss and other losses.
%Our proposed loss argues that the features extracted from the network should be able to predict its own category center. 
%We further proved the complementarity by plenty of experiments.
The results are shown in Table~\ref{tab:losses}. As seen, the incorporation of the CPL leads to consistent performance improvement in almost all cases. This clearly shows that the CPL is complementary to the other loss functions. 


%shows, our CPL can not only get good performance improvement by simply replacing the traditional metric losses, but also achieve higher performance by working together with the traditional losses.
%The $m=0.3$ in Triplet, and $m=0.4$, $\alpha=1.2$ and $T=10$ in RLL.
\begin{table}[tb]
    \begin{center}
    \scalebox{0.78}{
    \begin{tabular}{c|c|cc|c}
    \hline
    Projection &
      %\begin{tabular}[c]{@{}c@{}}Projection BN\\ (hidden)\end{tabular} &
      \begin{tabular}[c]{@{}c@{}}Target BN\\ (output)\end{tabular} &
      \begin{tabular}[c]{@{}c@{}}Predictor BN\\ (hidden)\end{tabular} &
      \begin{tabular}[c]{@{}c@{}}Predictor BN\\ (output)\end{tabular} &
      \begin{tabular}[c]{@{}c@{}}mAP (\%)\end{tabular} \\ \hline \hline
    No Pred. & $-$ & $-$ & $-$ & $85.59$ \\ \hline  
    $2$-layer Pred.             & $-$ & $-$ & $-$ & $85.40$ \\ \hline
    $2$-layer Pred.              & $\checkmark$ & $-$ & $-$ & $86.77$ \\ \hline
    $2$-layer Pred.              & $\checkmark$ & $\checkmark$ & $-$ & $\textbf{86.96}$ \\ \hline
    $4$-layer Pred.              & $\checkmark$ & $\checkmark$ & $-$ & $86.89$ \\ \hline
    $2$-layer Pred.            & $\checkmark$ & $\checkmark$ & $\checkmark$ & $86.59$ \\ \hline
    %Proj. ($3$-layer MLP) & $-$ & $\checkmark$ & $\checkmark$ & $-$ & $79.81$ \\ \hline
    %Proj. ($3$-layer MLP) & $\checkmark$ & $\checkmark$ & $\checkmark$ & $-$ & $80.59$ \\ \hline
    \end{tabular}
    }
     \caption{The influence of batch normalization in CPL on Market1501.}
     \label{tab:projection_BN}
    \end{center}
    \vspace{-5mm}
\end{table}

\paragraph{The influence of batch-normalization (BN) layers}
We find that using batch-normalization can make the training more stable and lead to improved performance. We compare the different ways of applying BN to CPL: (1) without applying BN to calculate the target (Target BN) (2) only applying BN for target calculation. (3) applying BN for both target calculation and Predictor $f(\cdot;\theta)$ (we test applying BN to different positions in the predictor). The results are shown in Table~\ref{tab:projection_BN}. As seen, the use of BN is beneficial. However, the benefit mainly comes from applying BN to target calculation. Whether apply BN to the MLP predictor has little impact on the performance.



%The architecture of our proposed CPL is similar to~\cite{chen2020exploring}, but the characteristics are different due to tasks difference.
%First, we remove all BN layers in the target and predictor, the performance is unsatisfactory whether there is MLP in CPL or not. And then adding BN at the output of the target can significantly enhance the performance.
%In a word, the BN layers are important in self-supervised methods, but it seems not so important in our loss, except the BN at target's output.
%The main reason for the differences may come from the differences of tasks.
%Our CPL is applied to supervised tasks, and is generally used together with softmax and other losses. At this time, there is no possibility of network collapse, and there is no serious optimization problem. Therefore, the influence of BN is not as great as that of self supervised tasks.


In addition, we also investigated the impact of the MLP structure. We test the performance by using a different number of layers in MLP. We find that the number of MLP layers in the predictor has little impact on the performance, and two layers are enough. Therefore, we choose a predictor with two layers, with its hidden node dimension as $512$.
%In self-supervised task, since there is no real label, the algorithm regards the same data with different augmentation methods as the positive sample pairs. If only positive samples are used in self-supervised learning, the network may fall into a trivial solution. 
%The projection is a $3$-layer MLP, its hidden node is $2048$-d. 
 %If there is no projection head, the projection output in the table is the output of the backbone.




==> Center Prediction Loss for Re-identification_arxiv/Introduction.tex <==
\section{Introduction}

Re-identification (ReID), as an important application of deep metric learning, aims to retrieve the images with the same identity of queries. The common solution is to construct an embedding space such that samples with identical identities (IDs) are gathered while samples with different IDs are well separated. To enforce such a property, loss functions that measure the quality of an embedding distribution plays a critical role and underpins the success of a ReID system.

Generally speaking, the loss function for ReID systems usually involves two terms: between-class discriminative losses and intra-class losses. The former encourages the separation of samples with different IDs, e.g., triplet loss \cite{schroff2015facenet}, ID entropy loss, circle loss \cite{sun2020circle} etc. Intra-class losses are applied to samples within the same ID, their main purpose is to reduce the intra-class variation of samples. For example, center loss \cite{wen2016discriminative} enforces all the intra-class samples to be clustered around a learned class-specific center.
It try to shrink samples of the same class into one point in the feature space and may easily drop their similarity structure~\cite{wang2019ranked}.
The empirical study shows that applying intra-class losses like center-loss can improve the generalization performance of learned metric in applications like face recognition \cite{wen2016discriminative}. However, for applications with higher intra-class variations like Person-ReID, 
%existing intra-class losses do not always lead to improved performance~\cite{luo2019bag}.
center loss can boost the clustering effect of features, but may reduce the ranking performance of ReID models~\cite{luo2019bag}.
This is because intra-class samples can exhibit significant intra-class variation and may not be characterized by a single center~\cite{sohoni2020no} or other existing simple distribution prior. 

\begin{figure}[tb]
\centering 
\includegraphics[scale=0.67]{figure1.pdf} 

%\end{minipage}}
\caption{An example illustrates the difference between the center loss and the center prediction loss. Assuming that the intra-class data distribution is a Gaussian mixture with two Guassian components, the center loss and center prediction loss incur different loss values. (a) For the center loss, since each data point is far from the center, a high loss value will be incurred. (b) For the center prediction loss, a point (red) far from the center can be mapped to a point close to the center of the remaining points through the learned MLP. Therefore, a much smaller loss will be incurred and more flexible similarity structure can be preserved inside the class. \textbf{Best viewed in color.}}
\label{fig:CPL_vs_center_loss}
\end{figure}


To overcome the issue of the current intra-class losses, in this paper we propose a new loss called the center prediction loss to strike the balance between intra-class variation reduction and flexible intra-class distribution modeling. The main idea is to regularize the intra-class data distribution via a simple requirement: a sample must be positioned in a location such that from it we can roughly predict the location of the center of remaining samples. The prediction error is treated as a loss function called center prediction loss. We show that using the predictor in the CPL allows more freedom in choosing intra-class distribution families and the CPL can naturally preserve the between-class discrimination. %In addition, we made a theoretical connection between CPL and the upper bound of entropy which measures the uncertainty of sample distribution.

%Thus minimizing CPL will reduce the uncertainty of sample distribution. Comparing with other center-based intra-class losses, e.g., center loss, our loss allows more flexible distribution formation since relatively small entropy can be achieved in multiple distribution families.   

By conducting extensive experiments on various person ReID and vehicle ReID datasets, we demonstrate the superior performance of the proposed loss and show that it can lead to consistent performance improvement to several existing ReID systems.

%With the recent widespread of video surveillance in public system, re-identification (ReID) has become a prevalent computer vision application, which aims at embedding visual appearance of various instances into an appropriate feature space where instances with identical IDs get gathered while ones with different IDs get separated with clear margins. The challenge lies in how to extract discriminative features and can generalize for identifying new unseen instances.

%ReID is an important applications of deep metric learning and constructing highly efficient loss function plays a key role in successful deep metric learning framework. 
%Center loss learns a center for features of each class and penalizes the distances between the features and their corresponding class centers. Pairwise losses such as contrastive loss learn the relationship between pairwise data points, and tripletwise losses such as triplet loss learn a distance metric by which the anchor point is closer to the similar point than the dissimilar one by a margin.
%However, most of these losses trend to pull data points in the same class as close as possible. They try to shrink samples of the same class into one point and may drop their intra-class distribution. ~\cite{luo2019bag} proved that higher intra-class compactness and inter-class separability on training set does not mean better performance on test set.
%To address this, RLL~\cite{wang2019ranked} propose to learn a hypersphere for each class. Specifically, instead of pulling intra-class examples as compact as possible, they force the distance of a positive pair smaller than a threshold, which is the diameter of each class’s hypersphere.
%But RLL does not consider that different classes have different intra-class  similarity structures and different distribution shapes. RLL uses a fixed threshold and sets the hyperspheres with same radius for each class to preserve the same degree of intra-class similarity structure.

%In this paper, we propose a new loss function, namely center prediction loss, to efficiently enhance the discriminative power of the deeply learned features.
%Our intuition is that if the feature extracted from a well trained network, it should be easy to predict its class center by a center predictor. 
%The CPL is applied on the features learned from the network. The center predictor used a $2$-layer MLP to predict the anchor's center. It maximizes the similarity between the predicted center and the mean of the rest positive features in the batch.
%Our loss can allow different classes to have different degree of intra-class similarity structure. Extensive experiments proved that the discriminative power of the deeply learned features highly enhanced by our CPL.



In summary, the contribution of this study is three-fold:
\begin{itemize}
\item 
We propose a new intra-class loss called \textbf{C}enter \textbf{P}rediction \textbf{L}oss (CPL). To the best of our knowledge, it is the first attempt to use the property of center predictivity as the loss function.

\item We show that the CPL allows more freedom for choosing the intra-class distribution family and can naturally preserving the discrimination between samples from different classes.
%make a theoretic connection between the proposed loss and an upper bound of the entropy of intra-class samples. 

\item Extensive experiments on various ReID benchmarks show that the proposed loss can achieve superior performance and can also be complementary to existing losses. We also achieve new state-of-the-art performance on multiple ReID benchmarks.
\end{itemize}

==> Center Prediction Loss for Re-identification_arxiv/RelatedWork.tex <==

\section{Related Work}
%\subsection{Margin-based Loss Functions}
%\subsection{Margin-free Loss Functions}
This section reviews some commonly used loss function for metric learning. 

\noindent\textbf{ID cross-entropy loss} treats each ID as an class, and use the cross-entropy loss to perform multi-class classification:
\begin{equation}
\mathcal{L}_{ce} =-\mathbb{E}_{\mathbf{x}} \left[ \log \frac{\exp \left(\mathbf{w}_{y}^{\top} \mathbf{x}+b_{y}\right)}{\sum_{j}^{C} \exp \left(\mathbf{w}_{j}^{\top} \mathbf{x}+b_j\right)} \right],
\end{equation}
where $\mathbb{E}$ is the expectation. $\mathbf{x}$ and $y$ are a randomly sampled embedding feature and its class label.  $\left[\mathbf{w}_{1}, \cdots, \mathbf{w}_{C}\right] \in \mathbb{R}^{d \times C}$is the weights of the classifier and $b$ is the bias term. In practice, we approximate the $\mathbb{E}$ with mini-batch in the SGD optimization.

% ## Center Loss ##
\noindent\textbf{Center Loss}~\cite{wen2016discriminative} simultaneously learns a center for each class and penalizes the distances between the deep features and their corresponding class centers.
% It's target is to make all samples as close to the center of their class as possible to increase the intra-class compactness:
%It aims to increase the distance between different categories and reduce the distance between the same class:
\begin{equation}
\mathcal{L}_{center} =\frac{1}{2} \mathbb{E}_{\mathbf{x}} \left[ \left\|\boldsymbol{x}-\boldsymbol{c}_{y}\right\|_{2}^{2}\right],
\end{equation}
where $\boldsymbol{c}_{y}$ is the learned center for class $y$. The definition of other symbols are same as above. 
% With the joint supervision of the ID cross-entropy loss and the center loss, center loss can get very good intra-class compactness and inter-class separability on the training set, but it doesn't mean high performance on the test set. In fact, in the ReID task, the center loss does little to improve the performance. Even sometimes it can cause performance degradation.
Working with the ID cross-entropy loss, center loss can obtain excellent intra-class compactness and inter-class separability on the training set. 
%However, for applications with higher intra-class variations like Person-ReID, center losses do not always lead to improved performance~\cite{luo2019bag}.
%However, center loss does not necessarily lead to improved performance on the test set, especially for many ReID tasks \cite{}. 

%but it doesn' high performance on the test set. In fact,sometimes the center loss can't make outstanding contribution to improving performance,even it will bring performance degradation to a certain extent in the ReID task.

% ## Triplet Loss ##
\noindent\textbf{Triplet Loss}~\cite{schroff2015facenet} applies to a triplet of samples called anchor point ($\mathbf{x}_a$), positive point ($\mathbf{x}_p$) and negative point ($\mathbf{x}_n$). It aims to pull an anchor point closer to the positive point (same identity) than to the negative point (different identity) by a fixed
margin $m$:
\begin{equation}
\begin{split}
\mathcal{L}_{tri}= \mathbb{E}_{\{\mathbf{x}_a,\mathbf{x}_p, \mathbf{x}_n\}}\left[
D(\mathbf{x}_a,\mathbf{x}_p) - D(\mathbf{x}_a,\mathbf{x}_n) + m\right]_{+},
\end{split}
\label{reward}
\end{equation}
where $D(\cdot)$ denotes euclidean distance, $m$ is a fixed margin and $[\cdot]_+$ is the hinge function.
%$m$ represents the minimum interval between the positive-pair distance and the negative-pair distance.
%From the definition of triplet loss, we can know that if the distance between the anchor and the negative sample is less than $m$, triplet loss will pull data points in the same class as close as possible like a center loss.

% ## Circle Loss ##
\noindent\textbf{Circle Loss}~\cite{sun2020circle} applies to a randomly sampled batch of samples. Given a single sample $\mathbf{x}$ in the feature space, assume that there are $K$ same-class samples which gives $K$ similarity scores and $L$ other-class sample which gives $L$ between-class similarity scores, then circle loss is defined as:
\begin{equation}
\resizebox{0.48\textwidth}{!}{
$\begin{aligned}
\mathcal{L}_{circle} 
%&=\log \left[1+\sum_{i=1}^{K} \sum_{j=1}^{L} \exp \left(\gamma\left(s_{n}^{j}-s_{p}^{i}+m\right)\right)\right] \\
&= \mathbb{E} \left[ \log \left(1+\sum_{j=1}^{L} \exp \left(\gamma\left(s_{n}^{j}+m\right)\right) \sum_{i=1}^{K} \exp \left(\gamma\left(-s_{p}^{i}\right)\right)\right) \right],
\end{aligned}
$}
\end{equation}
where $s_{n}^{j}$ is the intra-class similarity, $s_{p}^{i}$ is the between-class similarity. $m$ is the margin between $s_{n}^{j}$ and $s_{p}^{i}$ and $\gamma$ is a hyper-parameters.

% ## Lifted Structure Loss ##
\noindent\textbf{Lifted Structure Loss}~\cite{oh2016deep}
%is a loss function for taking full advantage of the training batches. The objective of this loss is to
tries to pull one positive pair as close as possible and pushes all negative samples farther than a margin $m$.
\begin{equation}
\resizebox{0.49\textwidth}{!}{
$
\begin{aligned}
\mathcal{L}_{LS}= \mathbb{E} \left[ \sum_{y_{i j}=1}\left(D_{i j}+\log \left(\sum_{y_{i k}=0} \exp \left(m-D_{i k}\right)\right)+\log \left(\sum_{y_{j l}=0} \exp \left(m-D_{j l}\right)\right)\right)_{+} \right],
\end{aligned}
$
}
\end{equation}
where $D(\cdot)$ is the distance metric, $ij$ is positive pair, $ik$ and $jl$ are negative pairs.

% ## RLL Loss ##
\noindent\textbf{Ranked List Loss (RLL)}~\cite{wang2019ranked} proposes to build a set-based similarity structure by exploiting all instances in the gallery. Different from the above methods which aim to pull positive pairs as close as possible in the embedding space,
%and the intra-class distribution might be dropped.
the RLL only needs to pull positive examples closer than a predefined threshold (boundary). In the form of pairwise constraint, the loss can be expressed as:
\begin{equation}
\mathcal{L}_{RLL}=\mathbb{E} \left[ \left(1-y_{i j}\right)\left[\alpha-d_{i j}\right]_{+}
+ y_{i j}\left[d_{i j}-(\alpha-m)\right]_{+} \right],
\end{equation}
where $d_{ij}$ is euclidean distance between $i$th sample and $j$th sample. $y_{i j}=1$ if $y_{i}=y_{j}$, and $y_{i j}=0$ otherwise. RLL aims to push its negative point farther than a boundary $\alpha$ and pull its positive one closer than another boundary $\alpha-m$. Thus $m$ is the margin between two boundaries.

% ------------------------------------------------
% ## N-pair-mc Loss ##
\noindent\textbf{N-pair-mc Loss} \cite{sohn2016improved} uses the structural information between the data to learn more discriminative features. Triplet loss pulls one positive point towards anchor while pushing a
negative one simultaneously. In the process of each parameter update, N-pair-mc loss also considers the relationship between the query sample and negative samples of different classes, prompting the query to maintain a distance from all other classes, which can speed up the convergence of the model.
%\begin{equation}
%\resizebox{1.0\hsize}{!}{$L\left(x, x^{+},\left\{x_{i}\right\}_{i=1}^{N-1} ; f\right)=\log\left(1+\sum_{i=1}^{N-1} \exp \left(f^{T} f_{i}-f^{T} f^{+}\right)\right)
%$}
%\end{equation} 
%The training samples is a $N+1$ tuple consists of  $x, x^{+}, x_{1}, \cdots, x_{N-1}$, $x^{+}$denotes positive sample relative to $x$, $\left\{x_{i}\right\}_{i=1}^{N-1}$ denotes negative samples relative to $x$, $f$ denotes function defined by deep neural network.

% ## Quadruplet Loss ##
%\textbf{Quadruplet Loss} is composed of triple loss, positive sample pair and relative distance loss. The latter enables the model to distinguish the relative distance between positive sample pair and negative sample pair. This part of the constraints can be understood as the minimum distance between classes is greater than the distance within classes
%\begin{equation}
%\begin{aligned}L_{quad}=\left(d_{a, p}-d_{a, n 1}+\alpha\right)_{+}+\left(d_{a, p}-d_{n 1, n 2}+\beta\right)_{+}\end{aligned}
%\end{equation}
%where $a$ is anchor, $p$ is positive sample, both of $n1$ and $n2$ are negative samples, due to $\left(d_{a, p}-d_{n 1, n 2}+\beta\right)_{+}$'s limitation, the inner distance should be greater than the inner distance.


%At present, face recognition methods are generally based on margin classification. Among them, margin appears in the form of $cos(m*theta)$. Will bring about the problem of too complex back propagation calculation. Coupled with a large number of hyperparameters to be processed, the impact on complexity is too large. \textbf{cosface loss} makes up for this defect.
%\begin{equation}
%L=-\frac{1}{N} \sum_{i=1}^{N} \log \left(\frac{e^{s\left(\cos \left(\theta_{y i}\right)-m\right)}}{e^{s\left(\cos \left(\theta_{y i}\right)-m\right)}+\sum_{j=1, j \neq y_{i}}^{k} e^{s \cos \theta_{j}}}\right)
%\end{equation}

%The design idea of itself is to subtract a positive value from the cosine space so that on the monotone interval of 0 - $\pi$ ,the $\theta_{y i, i}$ were affected well by $\cos \left(\theta_{y_{i}, i}\right)-m$ is samller than before,it indicates the angle between the sample and its own class center is too large.In order to improve the training environment of samples ,the variable m is Is added to the loss function.When loss converges, $\theta$ will be smaller and the class will be more clustered.

%\textbf{arcface loss} is an additive angular margin loss to obtain highly discriminative features for face recognition. It maximizes the classification limit directly in the angle space, while cosface maximizes the classification limit in the cosine space. This modification is because the angle distance has a more direct effect on the angle than the cosine distance.
%\begin{equation}
%L=-\frac{1}{N} \sum_{i=1}^{N} \log \left(\frac{e^{s\left(\cos \left(\theta_{y i}+m\right)\right)}}{e^{s\left(\cos \left(\theta_{y i}+m\right)\right)}+\sum_{j=1, j \neq y_{i}}^{k} e^{s \cos \theta_{j}}}\right)
%\end{equation}


%Not only the differences between the pre-defined samples are considered, but also the differences among all the samples in a batch. In this process, the paper introduces the idea of hard negative mining, considering the difficulty between positive and negative samples. In order to avoid the network training falling into the local optimal bug, the upper bound of loss function is introduced to alleviate this problem.

% ## MS Loss ##
%\textbf{MS Loss} is implemented using two iterative steps with sampling 5and weighting. it takes both self-similarity and relative similarities into account which enables the model‘s performance more efficient, which is formulated as,
%\begin{equation}
%\begin{aligned}
%L_{M S}=\frac{1}{m} \sum_{i=1}^{m} &\left\{\frac{1}{\alpha} \log \left[1+\sum_{j \in \mathcal{P}_{i}} e^{-\alpha\left(S_{i j}-m\right)}\right]\right.\\
%5+&\left.\frac{1}{\beta} \log \left[1+\sum_{j \in \mathcal{N}_{i}} e^{\beta\left(S_{i j}-m\right)}\right]\right\}
%\end{aligned}
%\end{equation}
%where $S_{i j}$ is the similarity between samples, $\mathcal{P}$ denotes positive samples and $\mathcal{N}$ denotes negative samples. $m$ is the fixed margin.
 

%With faster convergence and better performance in face recognition, center loss has been widely used in the existing re identification methods with no margin limited. 
%\textbf{group loss} uses the global information of the mini-batch to refine the local information provided by the softmax layer of a neural network. This iterative procedure categorizes samples into different groups, and enforces consistent labelling among the samples of a group. While softmax cross-entropy loss judges each sample in isolation,which formula can be expressed like followed:
%\begin{equation}
%X(t+1)=Q^{-1}(t)[X(t) \odot \Pi(t)]
%\end{equation}
\noindent\textbf{Limitations of the existing losses:} By analyzing the above loss functions, we identify the following limitations of the existing methods:
%From the above analysis of these loss functions, we can know that all of them have at least one of the following problems:
First, all of the above loss functions try to reduce the distance between samples of the same class. Most losses encourage the same-class samples to be shrunken into one point. However, this may hurt preserving the intrinsic intra-class sample diversity which has been shown to be beneficial for learning transferable features \cite{wang2019ranked}. 
%into one point and it may drop the intra-class distribution. It is not conducive to model learning more rich feature expression ability.
Second, some loss functions, such as RLL, use a fixed intra-class margin for all classes to regularize the intra-class sample distribution. However, a fixed margin can hardly be optimal for all classes.
%it ignores that the intr-class distribution of different classes is different, and the hyperspheres with the same radius are not the optimal solution.
%Third, many loss functions involves some hyper-parameters, e.g., margin $m$. Empirical study finds the choices of those hyper-parameters have an impact on the final performance. However, it might not be trivial to find a good set of hyper-parameters generalized to all

%most of these loss functions use margin to learn more discriminative features. Margin is a hyperparameter, and it is not easy to set the optimal margin w.r.t. different tasks and different datasets.
In contrast, our proposed CPL allows more flexibility in intra-class sample distribution and does not necessarily require same-class samples should have very small distances. Also, it does not involve any pre-set hyper-parameters and can be adaptive to each class. 


%is a margin-free loss function that uses the property of center predictivity to learn the discriminative feature, it can preserve intra-class data distributions with different shapes.

%\textcolor{red}{added by Lingqiao), we only need to focus on intra-class loss function. Do not need to list equations for all the loss functions}
